A Survey on Social-Physical Sensing: An Emerging Sensing Paradigm that Explores the Collective Intelligence of Humans and Machine

Propelled by the omnipresence of versatile data capture, communication, and computing technologies, physical sensing has revolutionized the avenue for decisively interpreting the real world. However, various limitations hinder physical sensing's effectiveness in critical scenarios such as disaster response and urban anomaly detection. Meanwhile, social sensing is contriving as a pervasive sensing paradigm leveraging observations from human participants equipped with portable devices and ubiquitous Internet connectivity to perceive the environment. Despite its virtues, social sensing also inherently suffers from a few drawbacks (e.g., inconsistent reliability and uncertain data provenance). Motivated by the complementary strengths of the two sensing modes, social-physical sensing (SPS) is protruding as an emerging sensing paradigm that explores the collective intelligence of humans and machines to reconstruct the "state of the world", both physically and socially. While a good number of interesting SPS applications have been studied, several critical unsolved challenges still exist in SPS. In this paper, we provide a comprehensive survey of SPS, emphasizing its definition, key enablers, state-of-the-art applications, potential research challenges, and roadmap for future work. This paper intends to bridge the knowledge gap of existing sensing-focused survey papers by thoroughly examining the various aspects of SPS crucial for building potent SPS systems.

==> architecture.tex <==
\section{Architecture of Social-Physical Sensing} \label{sec:architecture}
An architectural standardization is necessary to systematically address the challenges prevalent in SPS and provide a suitable abstract model for simplifying the design of future SPS systems, and provide a scalable yet robust environment to deploy SPS.

\begin{figure}[!htb]
    \centering
   \vspace{-0.05in}
    \includegraphics[width=8.5cm]{fig/arch.png}
    %\vspace{-0.05in}
    \caption{Architecture of SPS}
    \vspace{-0.1in}
    \label{fig:threedim}
\end{figure}

SPS is a rapidly developing sensing paradigm that harnesses the collective benefits of social sensing and physical sensing to absorb vital information from the environment around us. SPS provides a more effective information retrieval compared to standalone approaches by

\subsection{Components of Social-Physical Sensing}
\noindent\textbf{(Discuss the components of social physical sensing in general (i.e., the social sensing component with human ``sensors" and the physical sensing component with physical sensors (drones, cars, IoT devices, wearable sensors, etc.)))}

\noindent\textbf{(Explain how the two paradigms can complement each other (exploit the collective powers))}

\subsection{Variants of Social-Physical Sensing}

\noindent\textbf{(Introduce all the types of social-physical sensing. In particular: i) social-media-driven drone sensing (SDS), ii) social-media driven vehicular sensor networks (S-VSN), iii) integrated crowdsensing and IoT (Crowd-IoT) )}


\begin{comment}
\begin{table*}[!htb]
  \centering
  \caption{A Brief Summary of Representative SPS Application Paradigms}
  \scalebox{0.9}{
	\begin{tabular}{c||c||c||c}
\toprule
Scheme & Targeted Challenges& Objective & Solution Approach\\

\cmidrule(l){1-4}
    CollabDrone&i) Leveraging unreliable social signals to drive UAVs&Maximize Detection Accuracy&i) MLE-based Truth Discovery\\
    &ii) Identifying latent correlations among event locations&&ii) Spatiotemporal Correlation Inference\\
    &&&iii) Game-theoretic Task Allocation\\
     \cmidrule(l){1-4}
    SEAD &i) Conflicting objectives of event coverage versus energy&Maximize Event Coverage&i) MLE-based Truth Discovery\\
     &conservation &\&&ii) RL-based UAV dispatching\\
     &ii) Adapting to the dynamics of the social media and the &Minimize Energy Consumption&iii) Game-theoretic Task Allocation\\
     &physical world&&\\
     \cmidrule(l){1-4}
    SocialUAV&i) Leveraging unreliable social signals to drive UAVs& Maximize Detection Accuracy &i) Ensemble Truth Discovery\\
    & ii) Constraints from the physical world and social media&& i) Game-theoretic Task Allocation\\
    &iii) Developing a closed-loop system between social&& ii) Deadline-aware Path Planning\\
    &media and UAVs&&iii) CMAB-Based Social Media\\
    &&&Source Selection\\
    \cmidrule(l){1-4}
    CompUAV&i) Limited availability of social signals during forest fires&Maximize Fire Spread&i) Robust Truth Discovery\\
    &ii) Predicting the regions of fire where to dispatch UAVs&Prediction Accuracy&ii) CA-Based Fire Spread Prediction\\
    &&&iii) Game-theoretic Task Allocation\\
    &&&iv) Downhill Simplex Optimization\\
    \cmidrule(l){1-4}
    SM-MDT&i) & &i) \\
    \cmidrule(l){1-4}
        SocialCar&i) &&\\
    &ii) &&ii) \\
    &&&iii) Game-theoretic Task Allocation\\
     \cmidrule(l){1-4}
    DASC &i) &i) MLE-based Truth Discovery\\
     &conservation &\&&ii) Online MDP-based road damage discovery\\
     &ii) &iii) Game-theoretic Task Allocation\\
     &physical world&&\\
\midrule
\toprule
    \end{tabular}
    }
\label{tab:SPSsummary}
\end{table*}
\end{comment}

\begin{comment}

\subsection{Uncertainty Quantification in Social-Physical Sensing}

\subsection{Handling Communication Constraints During Disaster Scenarios}

\subsection{Energy-Aware UAV Dispatching for SDS}


\subsection{Mobility-Aware UAV Dispatching for SDS}

\subsection{Edge Computing and Federated learning for SDS}
In recent times, the advent of specialized yet inexpensive embedded hardware at the edge have opened new doors to perform complex computations locally withing the drones~\citep{majid2018shuffledet}. Thus, SAS can leverage the massive computation power of edge devices~\citep{shi2016edge}, providing unprecedented access to sensor data and processing power, enabling diverse applications such as object recognition, anomaly detection, survivor identification, and video analytics~\citep{sabokrou2018deep, casbeer2005forest}. In this paper, we explore the opportunity of exploiting the onboard hardware on UAVs for a comprehensive edge-based SAS framework. 

\subsection{Dynamic Incentive Management for S-VSN}

\subsection{Road Congestion Reduction for S-VSN}
\end{comment}


\begin{figure}[!htb]
    \centering
   %\vspace{-0.05in}
    \includegraphics[width=7cm]{fig/crowdiot.png}
    %\vspace{-0.05in}
    \caption{Overview of CrowdIoT Paradigm}
    %\vspace{-0.1in}
    \label{fig:crowdiot}
\end{figure}

%Existing privacy-aware sensing approaches in SPS tend to conceal sensitive attributes in the raw data before transmitting them to task managers for parameter tuning and model update. However, with the lack of crucial information such as names of places or geo-location tags, the critical events may not be located with sufficient accuracy, which may cause the SPS scheme to dispatch mobile agents such as UAVs to wrong locations. SPS applications often require the knowledge of locations from posted social media data which in conflicting with privacy requirements. Due to the strict privacy constraints from user devices (e.g., smartphones, wearables), an SPS application may not have unrestricted access to the user data. However, data analytics schemes in SPS (e.g., deep learning algorithms) inherently rely on training data for model updates. Without obtaining necessary information about the raw training data from clients, data-centric SPS applications tend to underperform or mislabel events from social media. For example, if sufficient data is not available, urgent events indicating location or survivors may be misclassified as false. The privacy and sensing quality trade-offs become more pronounced while concurrently considering the data modality and heterogeneity arising from multitudes of data generated by the social and physical sensors. One potential solution can be to incorporate federated learning (FL) that require training data to be stored locally and only accessible to the device owners with the goal of preserving privacy. While current FL approaches attempt to solve the potentially conflicting goals of preserving user privacy and maximizing sensing quality, they fall short in the context of SPS where the dynamics challenge also need to be considered. For example, batteries of smartphones may run out or there may be a sudden increase in the number of reported social media posts. Future research may focus on developing reliable FL models to better address the privacy and sensing quality concern.

%For example, a key assumption of existing fair ML is that the algorithmic bias is introduced by the “tyranny of the majority" - demographic groups with more training data often have lower error rates than demographic groups with fewer data [30]. Therefore, existing fair ML solutions often target at balancing the amount of training data of different demographic groups [5, 13, 20] to eliminate algorithmic bias. These approaches require access to either the raw training data or the underlying data distribution of the demographic groups, which are not allowed in our FL based problem setting. 

%Fairness and Performance Trade-offs: the third challenge lies in %
%One issue that arises when trying to ensure fairness and transparency in the distribution of input data is degradation of performance. In order to reduce the biasness, it is crucial to incorporate a wider distribution of data from different classes (e.g., race, ethnicity, nationality) of data contributors. However, this necessitates considering greater volumes of input data which may slow down the model update process. Existing schemes have attempted to reduce algorithmic biasness by manipulating the loss function of the model so that the training process of the model satisfies certain fairness constraints. The problem of such approaches is that they have been originally designed for input data whose accuracy is not questionable and is not applicable in the context of SPS where the input data is from the unreliable social media users who tend to pass misinformation and falsified claims. Thus, current approaches are not suitable for SPS applications to ensure fairness and transparency. The issue is made even more difficult due to the reliability and dynamic challenge prevalent in SPS. Thus, one potential future research direction can focus on balancing the fairness and performance of the data analytics algorithms involved in SPS. 

%For example, a random binary classifier has perfect fairness on a balanced dataset with a poor accuracy of the classification results (i.e., 50\% accuracy for both classes). The fairness and performance trade-offs become more complicated if the fairness of multiple demographic groups are considered simultaneously. For example, we found improving fairness of one demographic group may lead to the degradation of the fairness and accuracy of another. Consider a simple example where we have much more training data samples from males than females. To achieve fairness for the “female" demographic group, the model should be trained on a more balanced data by reducing the number of male data samples in the training process. However, if it happens that the male data samples are mostly African Americans, the data samples for them will decrease as well, leading to lower accuracy and potentially higher bias for the “African American" demographic group. It remains to be an open challenge on how to achieve a good balance between fairness and accuracy among different demographic groups. 

%The first approach is to remove/obfuscate the sensitive attributes in the raw data before training, making the trained model unaware of the demographic groups of the participants. However, such “unawareness" is not equivalent to “fairness", and often leads to biased models where some demographic groups have better prediction accuracy than others. The second approach is to manipulate the loss function of the model so that the training process of the model satisfies certain fairness constraints. However, these approaches are designed for training a single centralized model and not suitable for a distributed training environment. The third approach is to eliminate the data imbalance to ensure the ML model is trained on balanced data across all demographic groups. There exist many data sampling techniques  dedicated to addressing the data imbalance problem. However, they often require the knowledge of either the sensitive attributes of the data or the statistics of the raw data (e.g., distribution of “male" vs “female" data entries), thus violate the privacy constraints of the FL. In this paper, we propose a novel multi-agent reinforcement learning based scheme that ensures both the accuracy and fairness of the trained global model without accessing the private training data of clients.




%The first challenge refers to the restricted information that the server is allowed to access due to the strict privacy constraints of our problem. In particular, FL requires the training data to be stored locally and only accessible to the data owners (i.e., the clients) to protect their privacy. However, without accessing the necessary information about the raw training data of the clients, the FL server cannot apply current fair ML solutions to address the fair classification problem. For example, a key assumption of existing fair ML is that the algorithmic bias is introduced by the “tyranny of the majority" - demographic groups with more training data often have lower error rates than demographic groups with fewer data [30]. Therefore, existing fair ML solutions often target at balancing the amount of training data of different demographic groups [5, 13, 20] to eliminate algorithmic bias. These approaches require access to either the raw training data or the underlying data distribution of the demographic groups, which are not allowed in our FL based problem setting. Fairness and Performance Trade-offs: the third challenge lies in balancing the fairness and performance of the classification model learned by FL. It is well observed that reducing the bias (i.e., improving fairness) of the ML models often lead to the model performance degradation [4]. For example, a random binary classifier has perfect fairness on a balanced dataset with a poor accuracy of the classification results (i.e., 50\% accuracy for both classes). The fairness and performance trade-offs become more complicated if the fairness of multiple demographic groups are considered simultaneously. For example, we found improving fairness of one demographic group may lead to the degradation of the fairness and accuracy of another. Consider a simple example where we have much more training data samples from males than females. To achieve fairness for the “female" demographic group, the model should be trained on a more balanced data by reducing the number of male data samples in the training process. However, if it happens that the male data samples are mostly African Americans, the data samples for them will decrease as well, leading to lower accuracy and potentially higher bias for the “African American" demographic group. It remains to be an open challenge on how to achieve a good balance between fairness and accuracy among different demographic groups

%The first approach is to remove/obfuscate the sensitive attributes in the raw data before training, making the trained model unaware of the demographic groups of the participants [6]. However, such “unawareness" is not equivalent to “fairness", and often leads to biased models where some demographic groups have better prediction accuracy than others [35]. The second approach is to manipulate the loss function of the model so that the training process of the model satisfies certain fairness constraints [13, 36]. However, these approaches are designed for training a single centralized model and not suitable for a distributed training environment [24]. The third approach is to eliminate the data imbalance to ensure the ML model is trained on balanced data across all demographic groups. There exist many data sampling techniques [5, 20] dedicated to addressing the data imbalance problem. However, they often require the knowledge of either the sensitive attributes of the data or the statistics of the raw data (e.g., distribution of “male" vs “female" data entries), thus violate the privacy constraints of the FL. In this paper, we propose a novel multi-agent reinforcement learning based scheme that ensures both the accuracy and fairness of the trained global model without accessing the private training data of clients.

%One avenue for future research in SPS can be focused on addressing the dynamics and the data modality and heterogeneity challenge by incorporating adaptive AI models to effectively monitor the environment from the social and physical sensor data. To handle the huge volumes of multi-modal data that are generated by plethora of sensors that tend to vary widely in terms of heterogeneity, adaptive AI-based are required that can cater to the dynamically changing environment. Historically, AI models are built with a design philosophy that endorses centralized training and are non-adaptive to the environment\citep{zhang2019integrated}, due to which they may not be a viable approach for simultaneously handling the dynamics from the social and physical worlds. Thus, in order to analyze the obtained SPS data with adequate fidelity, expandable AI architectures need to be carefully designed that may be updated in real-time as the environment changes. With the growth of powerful edge devices (e.g., smartphones, IoT devices) and the demand for distributed model training over a large number of computing nodes, federated learning (FL) is gaining traction as a distributed AI training paradigm~\citep{konevcny2016federated}. In FL, a shared global AI model is trained from a collection of edge devices owned by end users, while retaining the training data within the edge devices~\citep{wang2019social}. By not transmitting the private data to a central server, FL manages to preserve user privacy and therefore foster trust among the participating users. The principle of FL aligns with our vision of scalable SPS systems by shifting AI from the cloud to edge devices. However, there are still outstanding challenges in FL that need to be addressed before establishing effective SPS schemes. One recurring issue in FL is the inconsistent availability of the edge devices, otherwise known as \textit{churn}~\citep{vance2019towards}. FL heavily relies on the participation of the edge devices for the training phase, which requires multiple iterations to converge to a global optima. Edge devices are owned by rational individuals who might abruptly leave in the middle of an ongoing AI model training process~\citep{wang2019social}. In addition to that, edge devices might periodically evict tasks for power savings, or may have a higher priority task to supplant the model training task, which may potentially negate the learning process and result in poor model parameter training~\citep{vance2019towards}. One limitation of many existing FL schemes is that they rely on synchronous model update operations~\citep{chen2019communication}. At every iteration of the model training, the server aggregates the model weights after receiving updates from all the clients. Due to the heterogeneity of the edge devices and the instability of network connections, all the devices cannot be guaranteed to have the same update interval~\citep{zhangedgebatch}. Thus, the server is prone to substantial downtime while needing to wait for all local updates before aggregation. In a time-sensitive SPS application, where deadlines are a crucial factor, such delays are undesirable. Therefore, it is an open challenge to simultaneously handle the churn issue and develop asynchronous model training in FL for scalable SPS applications.

==> unrelated.tex <==
 \begin{table*}[!htb]
  \centering
  \caption{Summary of highlighted SPS schemes according to categories}
  \scalebox{1}{
	%\begin{tabular}{p{4.5cm}||p{3.2cm}||p{5cm}||p{3cm}||c}
	\begin{tabular}{p{4.5cm}||p{3.5cm}||p{8cm}}
\toprule
Scheme & Data Acquisition Platforms & Roles of Humans in the System\\% & Challenges Targetesd & Area\\

\cmidrule(l){1-3}
    Social Airborne Sensing& Social Media+Mobile \& Fixed Physical Sensors&Share reports of individual health conditions and symptoms through social media.\\%&Data Collection, Security and Privacy, Human Interactions\\
    \cmidrule(l){1-3}
    Integrated social sensing and satellite-based remote sensing&Social Media+Mobile Physical Sensors&Augment satellite images by reporting the fine-grained activities on the Earth's surface.\\%&Data Collection, Data Modality and Heterogeneity\\
    \cmidrule(l){1-3}
    Anomaly detection using SAS and S-VSN&Social Media+Mobile Physical Sensors&Report Events and their corresponding locations on the social media to indicate anomalous events for dispatching UAVs.\\%&Data collection, Reliability, Dynamics, Human Interactions\\
    \cmidrule(l){1-3}
    License plate recognition using crowdsensing and physical sensors&Crowdsensing+Fixed \& Mobile Physical Sensors&Provide inputs through crowdsensing apps to track down plate number of a suspect's vehicle and find the whereabouts of the suspects.\\%&Data Collection, Reliability\\
    \cmidrule(l){1-3}
    Indoor localization combining social media sensing with IoT &Social Media+Fixed Physical Sensors&Deliver context information through social networking websites to locate them or objects they carry.\\%&Data Collection, Security and Privacy\\
    \cmidrule(l){1-3}
    Situational awareness using crowdsensing melded with IoT (CrowdIoT) &Crowdsensing+Mobile \& Fixed Physical Sensors&Collectively share data and extract information to measure, map, or predict processes of common interest.\\%&Data Collection, Data Modality and Heterogeneity\\
\midrule
\toprule
    \end{tabular}
    }
\label{tab:Scheme}
\end{table*}


%Advancements in sensor technologies have propelled physical sensors to transform into accurate and effective information acquisition tools that can sense occurrences in the physical world with high fidelity (e.g., dashboard cameras on vehicles, accelerometer on smartphones)~\citep{mitchell2014survey}. On the other hand, driven by the ubiquity of Internet connectivity and proliferation of portable devices, social sensing is an emerging sensing paradigm where reports on social data platforms (e.g., social news aggregation websites, crowdsourcing applications such as Waze) are analyzed to derive information about real-world events~\citep{wang2015social}. Although physical sensors have a proven reputation for reliably monitoring the environment, their sensing scope is vastly limited since: i) fixed physical sensors such as proximity sensors and surveillance cameras have to be set-up beforehand (e.g., over a road intersection) and cannot be transported to another location, and ii) mobile physical sensors (e.g., unmanned aerial vehicles (UAVs), vehicular sensors, smartphone) are restricted by battery life or are limited in number. Most importantly, physical sensors require some form of human assistance to locate events of interest regardless of being autonomous or not. By contrast, social sensing has greater sensing scope since it capitalizes on the pervasive nature social signals and the voluntary participation of individuals (e.g., any person possessing a smart device with Internet connectivity can post on the social media). However, since social sensing relies on the noisy social signals contributed by unvetted users, it suffers from inconsistent reliability, which restricts its usefulness in critical applications such as disaster response. 



%INTRO

%Fueled by the pervasive influence of human-centric sensing and the escalation of connected smart objects, social-physical sensing (SPS) is flourishing as a multifaceted sensing paradigm to acquire real-time information from the physical world~\citep{qiu2016integrating,de2017cyber}. SPS unifies the human-wisdom derived from social sensing with the empirical sensing capabilities of physical sensors to establish a comprehensive representation of the environment while minimizing their individual drawbacks (e.g, data reliability concerns of social sensing, limited range of physical sensor networks). According to recent statistics, it is estimated that there would more than 30 billion connected devices by the end of 2020~\citep{lucero2016iot} and as of January 2020, there are about 3.8 billion online social media users, which represents roughly 50\% of the world's population~\citep{kemp2020digital}.  %As of January 2020, 5.1 billion people had access to the Internet which represents about 66\% of the world's population, of which 3.8 billion constitute social media users~\citep{kemp2020digital}. 
%Thus, the confluence of social sensing's ubiquity (e.g., social media, crowdsourcing) with the versatile sensing capabilities of physical sensing devices (e.g., GPS, camera, thermal sensor) results in a definitive association of physical world observations collectively captured by the humans and physical sensors. A few notable application domains empowered by SPS includes urban search and rescue~\citep{dubey2019developing}, smart healthcare~\citep{chen2018urban}, wildfire monitoring~\citep{rashid2020compdrone}, simultaneous localization and mapping~\citep{jiang2019start}, human  mobility modeling~\citep{noulas2012tale}, and anomaly detection~\citep{lyu2016improved}. As SPS gradually permeates into our daily lives keeping human-in-the-loop (HITL), the lines between the social and physical realms rapidly turn blur. In this survey, we extensively study the underlying technology behind SPS, provide a rigorous overview of SPS along with different SPS schemes, and discuss the recurring challenges and opportunities in SPS. 



%Several existing survey papers have investigated sensing approaches that fall under the umbrella of cyber-physical-systems (CPS)~\citep{shi2011survey,mitchell2014survey,babiceanu2016big} and cyber-physical-social systems (CPSS)~\citep{de2017cyber,zeng2020survey,dressler2018cyber}. While these papers highlight a subset of SPS's features that intersect with CPS and CPSS and explore a few schemes that are partially related to SPS, they neither explicitly discuss the different paradigms enabled by SPS, nor provide an exhaustive summary of the state-of-the-art SPS schemes. Most importantly, past studies have overlooked the need for a standardized definition and an explicable overview of SPS, which is necessary to design, implement, and evaluate dependable SPS systems. In contrast to earlier survey papers, this survey presents a comprehensive overview of SPS, studies the key enabling technologies behind SPS, rigorously examines the different schemes driven by SPS, and scrutinizes the prevalent challenges in SPS as well as the avenue for future work to address the challenges.


%SPS is enabled by several major domains of technologies that includes data acquisition platforms (e.g., social media, vehicular sensors), computation paradigms (e.g., cloud and edge computing), and communication technologies and protocols (e.g., WiFi, LTE, and Bluetooth). %SPS capitalizes on a set of underlying technologies which includes the data acquisition platforms (e.g., social media, vehicular sensors), computation paradigms (e.g., cloud and edge computing), and communication technologies and protocols (e.g., WiFi, LTE, and Bluetooth). %SPS capitalizes on the technology developments in social sensing and physical sensing to generate corresponding digital representations of the involved physical entities. 


% explore a few SPS schemes that have evolved from these two domains

%The digital representation is used to derive knowledge about the state of the physical world and to optimize and control it through actions implemented through actuators. The related research area that is concerned with the integration of physical processes and computation in order to merge the physical and (IoT) paradigm, which seeks to interconnect computers to objects with self-configuring capabilities, plays an important role in the convergence of the physical and cyber worlds by ensuring secure and energy-efficient transfer of information (in both directions) between them. 

%At the forefront of
%necessity to interact with the physical environment
%The key technologies for designing CPSS relate closely to transdiscipline technologies covering CPS and CSS. Unfortunately, the design of CPSS is a complex task. First, CPSS are considerably complex systems due to the heterogeneity of network, complexity of software and the hardware entities, it lacks effective design approaches to systematically consider these issues in uniform. Second, the social part in CPSS still has not be received much attentions, there are not feasible approaches to uniformly model cyber, physical and social space. Finally, security issue has not been well investigated due that the CPSS are still in their infancy stage. Therefore, an effective, generic, security-critical design for CPSS is a challenging issue. To address this challenge, systematic design methodologies are needed to guide the effective design of CPSS. System-level design (SLD) methodology offers a promising way


%originating from machine learning, neural networks, federated learning, control theory, estimation theory, game theory, information theory, and distributed systems to mitigate the highlighted challenges. With the constantly changing environment around us, it is becoming increasingly important to develop compelling SPS schemes to sense the real-world phenomena.

%The first challenge exists in the data collection from the ensemble of innumerable social and physical sensors. The second challenge is transmitting the raw sensor data securely across different mediums and ensure user-level privacy. The third challenge constitutes handling the dynamics imposed by the social media reports and the physical world events. The fourth challenge lies in harnessing the unreliable social media data for dependable data analysis and extracting credible event reports to drive the physical sensors. The fifth challenge is the processing and interpretation of the massive volumes of data generated by diverse social and physical sensors and the heterogeneity of the different hardware involved in the sensing process. The sixth challenge is designing a closed-loop system to tightly integrate the social and physical domains.

%While the above challenges impose difficulty in developing effective SPS systems, they also set forth opportunities to instigate future research directions. We envision the potential to incorporate interdisciplinary techniques originating from machine learning, neural networks, federated learning, control theory, estimation theory, game theory, information theory, and distributed systems to mitigate the highlighted challenges. With the constantly changing environment around us, it is becoming increasingly important to develop compelling SPS schemes to sense the real-world phenomena. 


%\mt{\textbf{[TAHMID]}}


%\noindent\textbf{(Introduce Social Sensing (social media analysis, crowdsensing) and Physical Sensing (drones, vehicles). Talk about their individual strengths.)}

%\noindent\textbf{(Explain the key motivation behind integrating social sensing and physical sensing).)))}

%\noindent\textbf{(Elaborate the drawbacks of SS and PS and why it is important to integrate them (i.e., to exploit the complementary natures of each))}

%\mt{\textbf{[TAHMID]}}
%Highlight the key challenges in SPS. Challenges can be dirctly written from the Challenges section.

%\sk{\textbf{[SIAMUL]}}
%\noindent\textbf{(Provide an illustrative example of how SS and PS can be integrated (e.g, a set of tweets during disaster events that can be used to drive vehicles and cars to locations.)))}

%\sk{\textbf{[SIAMUL]}}

%\noindent\textbf{(Briefly detail the structure of the paper (i.e., a summary of all the sections).)))}

%Advancements in sensors and drone technologies are propelling autonomous UAVs to transform into agile and effective disaster response tools~\citep{erdelj2017help}. Autonomous UAVs utilize their on-board sensors (e.g., cameras,  infrared sensors) to identify event occurrences in the physical world (e.g., injured person on a roadside). On the other hand, due to the ubiquitous Internet connectivity and portable devices, social sensing is protruding as a new  sensing  paradigm where social media reports are analyzed to obtain information about the physical world~\citep{wang2015social}. A few notable examples of social sensing applications include detecting traffic abnormalities~\citep{zhang2018risksens}, tracking disease outbreaks~\citep{krieck2011new} and social unrest~\citep{al2014crowd}, and performing post-disaster damage assessments~\citep{danielicdcs18} using inputs from online social media (e.g., Twitter, Instagram, Facebook). 

%Although autonomous UAVs have proven their versatility in reaching a disaster location fast, a few limitations keep them from being widely adopted in real world disaster applications. One of these limitations is  the constant reliance on human inputs to provide guidance to the desirable locations, which induces delays in critical situations~\citep{richards2002coordination}. Moreover, UAVs operate on batteries or cells that provide only a finite amount of flight time~\citep{kim2016san}. With the onset of disaster scenarios requiring drones to continuously scan a large area over a long duration, the drones may fail to perform the tasks if they deplete their batteries~\citep{mohammed2014uavs}. 

%A drone is an expensive resource in the physical world that has to be utilized sparingly~\citep{mohammed2014uavs}. 


%\begin{figure}[!htb]
    %\centering
   %\vspace{-0.05in}
    %\includegraphics[width=6cm]{fig/threedim.png}
    %\vspace{-0.05in}
    %\caption{The three challenges prevalent in social-physical sensing}
    %\vspace{-0.1in}
    %\label{fig:threedim}
%\end{figure}




%\subsection{Reliability Challenge}
%  
%The integral constituents of SPS are the human-centric knowledge acquisition from social data platforms and the physical sensor data extraction from myriads of fixed and mobile sensors. The issue of reliability is emerges when simultaneously exploiting the social and physical sensors that have contrasting characteristics. Harvesting the social media data from the social data platforms involves filtering credible information from unreliable human sensors with unknown source reliability~\citep{IPSN:12} and as a result, a key issue lies in determining the authenticity of the reported events. Unreliable social media users are also known to provide falsified facts (i.e. misinformation) or rumors~\citep{R7} which, if not carefully discarded, might constrain the performance of the SPS system. Due to such uncertainty introduced by the unreliable social signals, administering the physical sensors becomes a serious issue, especially for time-sensitive applications like traffic risk identification or disaster response. For example, if unreliable social signals are used to send UAVs to purported locations where no actual events occurred, the SPS system would risk missing deadlines for critical events that actually exist. Additionally, SPS schemes typically use ground-based servers for processing raw sensor data which may be inaccessible in a disaster scenario if power lines and communication infrastructure become disrupted or unavailable (e.g., during a hurricane), reducing the reliability of the system. Several approaches have been developed to distill unreliable social signals such as estimation theory-based joint inference of claim truthfulness and user reliability~\citep{IPSN:12}, probabilistic technique-driven data quality improvement~\citep{yin2008truth}, and constraint-aware truth discovery~\citep{zhang2017constraint}. Despite their efforts, existing schemes solely rely on the noisy social media data to determine the veracity of claims posted on social media and do not integrate with any physical components for validating the ground truth or improving the estimation accuracy. Current schemes to address the reliability issue are tailored toward specific applications (e.g., anomaly detection or land usage classification) and not generalized. Moreover, exisiting approaches do not explicitly explore the impact of uncertain data quality that originates from human sensors on the social media. Thus, the reliability challenge at the unification of social and physical sensing remains an solved challenge in SPS.
 
%\subsection{Scalability Challenge}
%Several truth discovery solutions have been developed to mitigate the data reliability problem. For instance, Wang et al. presented a framework to jointly estimate the reliability of data sources and the correctness of the reported measurements in social media posts using approaches from estimation theory~\citep{IPSN:12,wang2014using}. Zhang et al. built upon the previous framework to address the scalability and physical constraint challenges and employed the improved schemes to real-world social sensing applications~\citep{zhang2018scalable,zhang2017constraint}. Yin et al. developed Truth Finder, a probabilistic algorithm using iterative weight updates to improve the quality of the data in social sensing~\citep{yin2008truth}. While great efforts have been made on developing reliable social sensing solutions, certain limitations hinder these solutions from being applied in SPS monitor the environment. One drawback of traditional social sensing schemes is that they solely rely on the noisy social media data and there no external means of validating the credibility of the input data~\citep{zhang2017constraint}. Hence, it remains an unresolved challenge in SPS to develop reliable social sensing models that can explore the uncertainty in the input data and extract reliable signals. 

%\noindent\textbf{(Elaborate on the problem of unreliable and noisy social media data contributed by unvetted human sources. Why is it difficult to drive drones/cars using unreliable signals? (e.g., drones might deplete their energy unnecessarily if sent to wrong locations; cars might be sent off to wrong locations; false alarms might cause rescue teams to be sent to wrong locations)} The second challenge lies in harnessing the noisy, sparse, and unreliable social ``signals" to develop dependable data analysis models for extracting credible event reports. 



%Combining Social Sensing with Smartphone and Fixed Physical Sensors for Healthcare Applications
    %Satellite-based remote sensing complemented with social media and crowdsensing
    %Anomaly Detection using Social Airborne Sensing (SAS) and Social Vehicular Sensor Networks (S-VSN)
    %Automatic license plate recognition (ALPR) using Crowdsourcing and Vehicular Sensors 
    %Indoor localization and Tracking by combining social media sensing with IoT 
    %Situational Awareness using Integrated Crowdsourcing and Internet-of-Things (CrowdIoT) 
    
    
    \begin{comment}
Table~\ref{tab:Challenges} provides an overview of the challenges in SPS.
\begin{table*}[!ht]
  \centering
  \caption{Prevalent Challenges in SPS Applications}
  \scalebox{1}{
	\begin{tabular}{p{3cm}||p{14cm}}
\toprule
Challenge & Description\\
\cmidrule(l){1-2}
    Data Collection&Locating, extracting, and organizing the raw sensor data from myriads of social and physical sensors dispersed throughout the world.\\
    \cmidrule(l){1-2}
    Security and Privacy&Transmitting raw data securely and ensuring personally identifiable information of online users does not stay at risk.\\
    \cmidrule(l){1-2}
    Dynamics&Adapting the SPS schemes to handle the constantly evolving social media reports and the events in the physical world.\\
    \cmidrule(l){1-2}
    Reliability&Filtering credible data from unreliable social media users with unknown source reliability to drive the mobile physical sensors.\\
    \cmidrule(l){1-2}
    Data Modality and Heterogeneity&Efficiently processing the huge volumes of data are generated by social and physical sensors every instant.\\
    \cmidrule(l){1-2}
    Human Interactions&Developing a closed-loop system that tightly integrates the social sensing and the physical sensing paradigms.\\
\midrule
\toprule
    \end{tabular}
    }
\label{tab:Challenges}
\end{table*}


    
    \begin{figure*}[!htb]
    \centering
   %\vspace{-0.05in}
    \includegraphics[width=16cm]{fig/challenges.png}
    %\vspace{-0.05in}
    \caption{Prevalent challenges in SPS Applications}
    \vspace{-0.1in}
    \label{fig:Challenges}
\end{figure*}
\end{comment}

%\mt{The growing number of connected devices in the real-world with sensitive data necessitates secure and accessible data sharing that allows SPS applications to harness the required information effortlessly without exposing any identifiable traces. In diverse networks consisting of innumerable social and physical sensors, ensuring security and accessibility simultaneously is a non-trivial task. To maximize security, the availability of information has to restricted, which might cause poor accessibility to data in an SPS system. On the other hand, to maximize accessibility, an SPS system has to give up security. Thus, careful consideration has to be taken to strike an efficient trade-off between security and accessibility. The core functionality of SPS is based on the exchange of information between a huge number of connected sensors. One perennial problem that has not been solved entirely by existing literature is the security of different data transfer protocols in SPS~\citep{toch2012personalization}. As such, securing data exchange is necessary to avoid potential security vulnerability and flaws while establishing confidence among users to contribute data. It is yet to be determined how to develop robust privacy-aware SPS platforms that can address the security and privacy challenge in SPS.} 

%an real-world events might be located in regions that are physically very far away from one another (e.g., different cities) and associated with contrasting deadlines based on their urgency (e.g., a traffic congestion vs. a critically wounded person)~\citep{zhang2017constraint}. Moreover, during a natural disaster (e.g., flood or hurricane), roads could become disconnected due to damage, hindering the movement of ground units such as cars and UGVs. In addition to that, UAVs have varying flying speeds depending on their battery health and physical environments (e.g., winds). The above factors from the physical world further exacerbates the problem of handling the dynamism of the social media. Therefore, careful consideration must be given to adapt the resource management strategy to accommodate these dynamics on-the-fly. 

 %and a resource management strategy that might have been successful when there were a few events concentrated nearby might not be ideal for a case where the events become scattered and located far away

%\mt{The social world events might have a causal effect on the physical world occurrences.}


--------------------------------------------------------------------------------------
%Application Section


%Figure~\ref{fig:SAS} illustrates the working principle of representative SAS schemes.

%\begin{figure}[!htb]
    %\centering
   %\vspace{-0.05in}
    %\includegraphics[width=8cm]{fig/sas.png}
    %\vspace{-0.05in}
    %\caption{Overview of the SAS Paradigm}
    %\vspace{-0.1in}
    %\label{fig:SAS}
%\end{figure}

%An S-VSN scheme called SocialCar has been developed which uses an incentivized social media-driven  task allocation approach for VSNs in smart city applications such as anomaly detection, risky traffic location identification, and environmental monitoring~\citep{rashid2019socialcar}. SocialCar attempts to jointly address the reliability challenge and the human-interactions challenge by leveraging a top-down incentive control mechanism to dynamically adjust the incentives for exploration of the event locations based on the aggregated reputations of the cars. 

%After a disaster such as hurricane, road damages are evident which disconnects road networks, causing the dynamics challenge in SPS. A damage-aware S-VSN scheme called DASC has been developed which addresses the dynamics challenge by using a Markov Decision Process (MDP)-based damage discovery scheme to locate roads affected by damage and use the obtained knowledge to make optimal route planning decisions.

%To address the dynamics and reliability challenges in SPS, a SAS approach called CollabDrone has been developed that identifies latent correlations among event locations to drive UAVs to regions of interest~\citep{rashid2019collabdrone}. By incorporating a spatiotemporal-aware inference model to compute the temporal, contemporaneous and lagged spatial correlations of prior and concurrent event locations, CollabDrone achieves a satisfactory degree of detection accuracy by selectively dispatching only a small number of UAVs.

%One important concern in SAS is addressing the dynamics challenge through careful management of UAVs to cater to their individual energy constraints and maximize detection accuracy. An energy-aware SAS scheme called SEAD has been developed that uses a reinforcement learning-based drone dispatching strategy to adapt to the physical and social environments and launch an appropriate proportion of UAVs for event exploration optimizing detection accuracy and energy consumption~\citep{rashid2019sead}.

%Urban search and rescue (USAR) missions require careful collaboration between various ground and remote teams to locate potential survivors. A SAS scheme called SM-MDT has been developed that uses social-media signals for tasking drone swarms in USARs. SM-MDT utilizes graph traversal algorithms to incorporate social signals for planing rescue missions and identifying search tasks.

%A SAS scheme called SocialDrone has been developed to address the reliability and human interactions challenge in SPS. SocialDrone leverages social media signals to drive UAVs to target areas to validate the truthfulness of emergency events~\citep{rashid2020socialdrone}. A closed-loop source selection mechanism uses the validation results from the UAVs to dynamically filter out unreliable users on social media which helps in improving the event detection from social media data by minimizing the chance of falsified claims.

%Wildfires are costly natural phenomena and monitoring the propagation of wildfires is an important step for suppressing such a calamity. An enhanced SAS scheme called CompDrone has been developed for monitoring wildfires that exploits the collective strengths of computational wildfire modeling and SAS by leveraging techniques from cellular automata, constrained optimization, and game theory~\citep{rashid2020compdrone}. 

%In the following subsections we discuss the state-of-the-art SAS schemes.

%In contrast to standalone UAV and social sensing, SAS approaches are more empirical as they capture real-world observations using physical sensors on UAVs, and have wider scope due to their reliance on human inputs from social data platforms. 


%\mt{user feedback}
%Likewise, depending on the application context, a SAS might be more practical than an S-VSN is a few cases, especially when road networks are entirely unavailable (e.g., searching for survivors during a forest fire or damage assessment after a hurricane). 

subsubsection{\mt{Social airborne sensing (SAS)}}
%\noindent\textbf{(Explain why it is important to determine the correlation between the events (i.e., to reduce travel of the UAVs, save time, etc.), discuss the challenges, how CollabDrone solves the challenges, briefly explain the solution approach)}


%The composite correlation inference model dynamically identifies the events from prior and concurrent events, and selectively dispatches UAVs by exploring the identified correlations. The key distinction of the CollabDrone with other SAS schemes lies in its analysis of the different correlations between the events in the real-world.

%\subsubsection{SEAD Framework}
%\noindent\textbf{(Explain why it is important to manage the tradeoff between energy conservation and event coverage (i.e., to minimize dispatching of the UAVs and prevent UAVs from running out of charge), discuss the challenges, how SEAD solves the challenges, briefly explain the solution approach)} % Additionally we develop a reinforcement learning-based energy-aware UAV dispatch strategy to selectively send out UAVs to event locations. iii) How to adapt to the constantly evolving social media where the social media users are highly dynamic. 
%Such requirements give rise to the potentially conflicting goals of maximizing event coverage and minimize energy consumption.  SEAD further uses a game-theoretic UAV task allocation approach to steer the UAVs to the locations where the social signals are uncertain and verify the event information extracted from unreliable social media data. 

%\subsubsection{SM-MDT Framework}
 %\noindent\textbf{(Discuss the paper by Terzi, Maria, Panayiotis Kolios, Christos Panayiotou, and Theocharis Theocharides. \textit{``Towards a Social-media Driven Multi-UAV Tasking platform"})} As elaborated in this work, social-media are a source of timely and valuable information regarding the occurrence, the evolution and the damageIn this work a novel multi-drone search and rescue framework is developed that considers social-media signals in the creation of search tasks. The key design challenges of implementing the proposed framework are discussed and a simulated scenario based on a real-life Twitter data set is presented as a means of providing evidence of the effectiveness of the proposed framework. produced in disasters.

%\subsubsection{SocialDrone Framework}
%% To address this problem, we develop a closed-loop source selection technique to utilize the verified information obtained by the UAVs to filter out unreliable users in the social sensing. % The integration of the cyber, physical and social realms can thus enable unprecedented dimensions of sensing with immense scope and reliability.\noindent\textbf{(Explain why it is important to selectively discard unreliable social media users over sensing cycles, discuss the challenges, how SocialUAV framework solves the challenges, briefly explain the solution approach)}
%As discussed in the reliability challenge in SPS, unreliable social media users tend to report misinformation or falsified claims which subsequently yields the human-interactions challenge (e.g., response teams relying on misinformation to make their decisions). It is important to selectively discard unreliable social media users over sensing cycles, discuss the challenges. 
 
%\subsubsection{CompDrone Framework}
%\noindent\textbf{(Explain why it is important to predict wildfires and integrate SAS with computational modeling, discuss the challenges, how CompUAV framework solves the challenges, briefly explain the solution approach)} Traditionally computational models have been used to predict wildfires and are known to provide reasonable accuracy.

%Figure~\ref{fig:svsn} shows an overview of the S-VSN paradigm.
%\begin{figure}[!htb]
    %\centering
   %\vspace{-0.05in}
    %\includegraphics[width=8cm]{fig/SVSN.png}
    %\vspace{-0.05in}
    %\caption{Overview of the S-VSN Paradigm}
    %\vspace{-0.1in}
    %\label{fig:svsn}
%\end{figure}

%\subsubsection{SocialCar Framework}
%\noindent\textbf{(Explain why it is important to use the existing road network, discuss the challenges, how SocialCar solves the challenges, briefly explain the solution approach)}

%(i.e., the historical behavior of the cars in attempting to successfully complete the tasks).

%\subsubsection{DASC Framework}
%\noindent\textbf{(Explain why it is important to consider the road damage along the routes (also may discuss the limitation of the SocialCar framework), discuss the challenges, how DASC solves the challenges, briefly explain the solution approach)}
 %DASC is the first S-VSN solution that connects the realms of social sensing and VSNs with explicit consideration of road damage.
%While substantial effort has been contributed to develop reliable SAS schemes, a few open research questions still exists in SAS which include : i) how to leverage the noisy and sparse social media signals to guide UAVs to anomaly prone locations? ii) How to accommodate various constraints imposed by the physical world (e.g., meeting the deadlines of urgent events, conforming to the constraints on the number of available UAVs and their flight time limited by the battery capacity)? iii) How to leverage the measurements collected by the UAVs to improve the social sensing process? A multifaceted SAS system is yet to be developed to address these questions.
%\noindent\textbf{(If other papers on SAS are found, discuss them as well and update Table 1 accordingly)}
%\noindent\textbf{(Introduce the summary presented in Table 1. Compare and contrast the schemes briefly (e.g., can discuss which approach may be suitable for which scenario))}
%\paragraph{Test Modified Paragraph}
%\subsection{B2}
%\paragraph{D1}
%\subsubsection{C2}
%\noindent\textbf{(Elaborate on each of CollabDrone, SEAD, SocialUAV, CompUAV and other frameworks)}


%\subsection{Augmented Virtual Reality by Combining Crowd Sensing and Social Data Mining with large-scale Simulation}
%With the increasing trend of augmented reality applications, the need for robust situational awareness tools are spiraling~\citep{bosse2019augmented}.

%just keeping the description here, if you think this belongs in the indoor localization section keep it, this is indoor localization with mobile sensors though doesn't really fall under localization + social media. (for location based services)

%\noindent\textbf{(Introduce the CrowdIoT platform in general)}\\ %Recently, advances in Crowdsensing is creating opportunities for new forms of experimentation in the area of IoT. 

%They define ``Susceptible (S)'' as people who are in disaster area but are not trapped, ``Infected (I)'' as people who are trapped in a certain spot, and ``Recovered (R)'' as people who are dead. They reason that people in the disaster area with social media access will provide information about themselves on social media to increase the likelihood of their survival and, as such, this crucial information such as their location can be obtained by monitoring their social media. They propose to provide IoT equipment in rescue packages which will aid people from the ``S'' class to increase their search radius and share their supplies with others.

%Trottier presented an exploratory overview of crowdsourced surveillance of closed-circuit television (CCTV) footage over the Internet \citep{trottier2014crowdsourcing}. They elaborated upon four existing crowdsourced CCTV surveillance websites: Crimestoppers UK, Facewatch, Internet Eyes and Shoreditch Digital Bridge to explain the emerging phenomenon of how crowds can be integrated into CCTV surveillance, ranging from identifying suspects to designating suspicious behaviour in everyday activity


--------------------------------------------------------------------------------------
%Challenges Section
% and \mt{relating the collected data to one another across the sensing paradigms}~\citep{stieglitz2018social}.
%Therefore, the noise originating from the social and physical sensors in SPS applications adversely affect the performance of one other causing difficulty collecting clean sensing data. } %For example, in a road damage detection application where the sites of road damage are determined using satellite images while human observations through crowdsourcing apps are used to further acquire the fine-grained location and severity of the damage (e.g., finding an exact street with damage), low resolution satellite images might yield incorrect areas of damage, sending the human sensors to wrong places. Conversely, unreliable human sensors might incorrectly report the extent of the road damage in the crowdsourcing app, resulting in poor damage severity analysis. Thus, the noisy social and physical signals cumulatively make it difficult to  reliably acquire knowledge in SPS applications.} %and the severity of the road damage is obtained using human observations on a crowdsourcing app, errors in GPS signal might result in incorrect road damage locations while unreliable human sensors might incorrectly report the extent of the road damage. These noises generated from the physical and social channels together make it difficult to locate the damage site and assess its severity. %Low resolution images from satellites might not reveal the exact location of a damage, sending social sensors to incorrect locations. Conversely social media users might report a wide range of ``damage" on social media websites (e.g., property damage, collateral damage) and not just road damage, making it difficult to determine the extent of the road damage. %For example, in the road damage detection application in Figure~\ref{fig:block}, people might report a wide range of ``damage" on social media websites (e.g., property damage, collateral damage) and not just road damage, making it difficult to locate the actual road damage. At the same time, the image captured by the satellites might not be able to capture the fine-grained extent of the road damage due to limitation of the image resolution. Without properly locating the road damage site and determining its extent, the damaged roads might not get repaired.
%In addition to that, current solutions overlook the fact that sufficient social and physical sensing data might not be available in the first place due to several reasons: i) social sensing APIs are known to impose certain limitations (e.g., rate limitation on crowdsensing apps like Waze) and social sensing data might be deleted by the users or the websites~\citep{zhang2019deeprisk,makice2009twitter}; and ii) the coverage of physical sensors might be limited (e.g., in a large city, surveillance cameras might not be able to cover every part).} %Therefore, collecting raw sensor data from the social and physical realms that direct to the appropriate information remains an open challenge in SPS.}



%\mt{unstructured and diversified information contained in both social and physical sensing platforms.}
%For example, after the onset of a \mt{disaster like a building on fire}, if keyword-based searches are executed to filter data from social data platforms using terms like ``fire" and ``smoke", the resulting posts might indicate unwanted incidents like ``fire ants marching" or ``smoke from a car exhaust". \mt{Moreover, given the huge number of physical sensors (e.g., the building on fire might have hundreds of IoT-based smoke detectors on each floor), it might become difficult to decide which subset of sensors to select and prioritize in an SPS application.} In addition to that, human sensors tend to inject sarcasm with their observations which makes the data collection process even harder \mt{(e.g., there might not be a real fire in the first place).} 
%\mt{While existing research have presented solutions to locate useful data from social and physical sensing platforms individually using statistical and data driven approaches ~\citep{nur2015combination,zhang2018light,jagannatha2016structured}, \mt{when the two paradigms are integrated such solutions are inadequate since they ignore interdependence of the social and physical data. It is crucial to relate the collected social and physical data to each other to accurately perceive real-world occurrences. For example, in a}} \mt{approaches like  they are still inferior to human perception in pinpointing useful social media data. }While existing research have presented solutions to detect sarcasm using statistical and machine learning approaches, %approaches like singular value decomposition (SVD)-based K-means clustering~\citep{nur2015combination}, adaptive sampling~\citep{zhang2018light}, and recurrent neural network (RNN)-based text labels~\citep{jagannatha2016structured}, they are still inferior to human perception in pinpointing useful social media data. Such interdependent noise originating from the social and physical data platforms cause difficulty in cleanly collecting sensor data.

%Amazon  %While such approaches might work for networked devices, they are hard to be applied to online users primarily because human behavior is hard to model and predict. For example, even after allocating incentives to sensing tasks in a VSN, the car drivers might still not be willing to carry out the tasks (e.g., when there is risk associated with the travel). 

%\mt{The design of such a closed-loop system requires a careful coordination of the interactions between the social and physical worlds, both of which are highly volatile. For instance, the number of human sensors contributing knowledge and their reliability might change infrequently over time~\citep{zhang2018scalable}. The truthfulness of the reported claims by the human sensors on social data platforms might also evolve steadily. Similarly, the events in the physical world might spontaneously occur at different locations and have varying degrees of urgency. For example, an event indicating an injured person might have a greater urgency than an event indicating a road closure~\citep{zhang2017towards}. Consequently, every event might have a deadline based on its corresponding urgency.} 

%\mt{In addition to the above, widespread prevalence of rumors and misinformation can lead human sensors to being overly sensational or biased in expressing their opinions in the social data platforms~\citep{kim2016garbage}. This nature of human interaction can potentially trigger misrepresented or misinterpreted observations and potentially lead to failures of physical sensors. For example, in the anomaly detection application in Figure~\ref{fig:block}, if the person posts a false claim on social media, the UAVs might be dispatched unnecessarily, depleting battery life. Another critical difficulty stemming from the human aspect of SPS is deciding how to handle the reaction of human sensors when an abnormal event occurs (e.g., a political unrest). It is also imperative to model how people react to the information contributed to them by their associates and acquaintances. Therefore, it entails a tight integration and collaboration between the social domain and physical world where social sensing and physical sensing complement each other. For example, the wide coverage of social signals can be used to complement the accurate sensing capability of physical sensors. The closed-loop challenge at the intersection of the physical and social spaces remains an outstanding challenge in the way of constructing reliable SPS systems.} 

%\mt{Although humans are a crucial component of SPS, they are also one fundamental point of failure in SPS. Recent studies have explored human-centric approaches that have the design philosophy of placing humans in the control loop with the intention that users might retake control of their information. This could potentially lead to the design of novel crowdsourced and socially informed architectures where users control the links of their networks. However, before realizing the potential of such approaches, novel and innovative forms of human-centered applications need to be developed to first resolve the human interactions challenge in SPS. } %As such, managing the interplay between the end-users, the devices they interact with, and the environment within an integrated paradigm consisting of social sensing and physical sensing requires close collaboration and communication between these facets.}



%A few examples of such devices are: i) smartphone sensors, thermostats, speed radars, proximity sensors, and optical sensors for data acquisition; ii) 5G LTE modems, Wi-Fi routers, network interface cards, and Bluetooth receivers for communication; and iii) GPUs, CPUs, quantum processors, FPGA, AI accelerators, and micro-controllers for data processing. Due to the inevitable complexities of catering to the individual characteristics of such diverse devices in the presence of social and physical signals, it is arduous to orchestrate them for collectively performing the different stages of sensing tasks in SPS applications. 

% many of these devices carry out tasks that are interdependent (e.g., multiple devices in a pipeline might carry out several stages of image processing), which the current approaches might break; and iii) many SPS applications have complex hardware requirements which current solutions do not account for (e.g., an anomaly detection application might require deep learning libraries on a processing device).} %and iv) SPS applications chiefly rely on mobile devices with limited power budgets and the processing overhead added by existing solutions might rapidly deplete their batteries.}

%\mt{Refining and interpreting meaningful information from colossal volumes of data generated by the social and physical sensors is a non-trivial task. Due to the diversity and large number of various sensing devices involved in social and physical sensing, it is imperative to design a system that can process the rapidly generated incoming signals in an efficient and timely manner~\citep{wang2015social}. Such devices also typically generate signals which are often unstructured and consists of multiple attributes and features. The types of data can widely vary across as text, image, location, audio, and video~\citep{birke2014big} and each type can further encompass different dimensionality as well which makes the processing even harder.} %Each type of sensing device (e.g., an IoT-enabled thermostat, a dashboard camera) typically has its own access control mechanism (i.e., authentication methods such as passwords and access tokens), communication protocol, and application programming interface (API), which makes it virtually impossible to rely on a single method for integrating all of them.} 

%\mt{Given these complexities arising from the data and device heterogeneity in SPS, data processing solutions need to be developed which can withstand this diversity in data and device characteristics and conclusively extract information. Moreover, since multi-modal data processing intrinsically demands greater compute power, care must be given to efficiently strike a trade-off between detection accuracy and computational complexity. A set of unsolved questions springing from the data modality challenge in SPS are: i) How to efficiently fuse the different types of social media data into one unified data stream? ii) How to design algorithms to process a wide variety of social data in real-time for an accurate detection of real-world occurrences? iii) How to speed up the analysis of multi-modal data for faster event discovery by distributing the computation across multiple devices? Due to heterogeneity of the different hardware and their generated data incorporated in the SPS, a unified scheme to manage them efficiently is yet to be designed.} 

%\mt{In SPS a major difficulty exists in processing the rapidly generated incoming physical and social signals consisting of diverse features or dimensions~\citep{wang2015social}. This challenge is identified as \textit{data heterogeneity} in data science research where large amounts of unfiltered and unstructured data with multiple modalities need to be processed~\citep{chu2016data,zhang2019transland,zhang2020trans,shang2019towards}. Specifically, data heterogeneity refers to the different variety or types of data prevalent in the social media such as text, image, location, audio, and video~\citep{birke2014big}. Moreover, each type can further encompass different dimensionality as well which makes the data heterogeneity challenge even harder.} 

% during a search and rescue mission, an UAV might be processing images using its onboard computation hardware and might not be able to simultaneously capture images and transmit the images, while an user might. } %However, those efforts have not established sufficient confidence among individuals to share their sensor data. }  %Moreover, given the large number and variants of available sensors on \mt{personal devices}, selecting the correct sensor for a particular SPS application is also an arduous task. 
% Several sensors might point to the same set of information, inducing redundancy. 

% Current research to study the correlation within social data platforms include methods such as semantic pattern recognition~\citep{dey2018fake}, graph mining-based social network centrality analysis~\citep{lutu2019using}, trust and influence modeling~\citep{asim2019trust}, deep auto-encoding and neural word embedding~\citep{zhang2018fauxbuster}. On the contrary, physical sensors do not typically inherit any such correlation and are more likely to be independent (e.g., two air quality monitors are unlikely to propagate the error of one another). Several efforts have studied ways to model the independence in physical sensors through sensor networks and mathematical models~\citep{ahn2011new,li2007connection,kim2018development}. Current knowledge discovery and data mining approaches in social and physical sensing assume model the  correlations across social and physical data platforms independently. However, when the social and physical sensors are combined together in SPS, existing approaches are limited in addressing the dependency and correlation challenge to collectively sense the real-world stimuli. It requires careful scrutiny of the data and accurate data provenance approaches to identify and characterize the spatiotemporal correlations. For example, } 

%First, across social sensing platforms, human sensors sensors tend to be naturally correlated (e.g., followers in Twitter are inclined to re-tweet the reports of their friends), which makes it relatively intuitive to model and analyze. %Understanding the dependency between peers in social data platforms in SPS can potentially eliminate biases and increase the quality of contributed knowledge. Current research to study the correlation within social data platforms include methods such as semantic pattern recognition~\citep{dey2018fake}, graph mining-based social network centrality analysis~\citep{lutu2019using}, trust and influence modeling~\citep{asim2019trust}, deep auto-encoding and neural word embedding~\citep{zhang2018fauxbuster}. On the contrary, physical sensors do not typically inherit any such correlation and are more likely to be independent (e.g., two air quality monitors are unlikely to propagate the error of one another). Several efforts have studied ways to model the independence in physical sensors through sensor networks and mathematical models~\citep{ahn2011new,li2007connection,kim2018development}.} There might be indirect connections which might explain the to latent features (e.g., distance between the gas stations or the supplier of gas at the stations).

%\mt{In contrast to social sensors which predominantly consists of humans, the deployment complexity and cost of physical sensors might require greater manual effort and financial provisions. In SPS applications with scarce resource availability and budget constrained, such deployment complexity and cost might not be feasible. If the spatiotemporal correlations between the social and physical data can be derived and exploited, they can be used to potentially lower the burden from physical sensors. For example, in the contact tracing application in Figure~\ref{fig:block}, if a strong spatiotemporal correlation in identified between the data provided by the wearable sensors and the people's posts on social media platforms, the number of required wearable sensors could be reduced.}

%However, given the inherent dependency across the social and physical sensing paradigms, existing solutions are unable to explore the underlying correlations and construct an unified framework for leveraging the correlations for a holistic representation of the environment. } %and require careful scrutiny of the underlying features While using such  correlations provide greater efficiency in the deployment of SPS applications, studying such intricate correlations across data form two distinct sensing domains is not a trivial task. 

%\mt{Thus, it is imperative to design } 

%For instance, in the crime reporting application in Figure~\ref{fig:block}, the social sensors might be interdependent on each other and propagate misinformation or rumors like falsely reporting the location of a crime. When these social signals are used to augment the WSN for locating a suspect, it might yield erroneous information about the whereabouts of the suspect.

 

%mainly because of the intrinsic difference and incompatibility between the social and physical %\mt{Once raw data is obtained from the different sensors in SPS, it is imperative to relate them to one another for obtaining a holistic representation of the situation. For instance, in a crowdsensing app and roadside sensors based traffic risk identification application, people might report about accidents through the crowdsensing app at a certain segment of a road and the roadside sensors might detect the speeds of cars crossing the segment. If the two data are related to each other, it might help to identify the segment of the road prone to greater traffic risk.}

%\mt{When the social and physical sensing paradigms are tightly integrated, it is imperative to study the relation between the sources and the data derived from each paradigm. As such, one pivotal challenge in SPS is determining how to characterize the dependency and correlation between the data sources upon melding physical and social sensors in a closed context.}

%\mt{Across social sensing platforms, it has been observed that human sensors tend to follow the views and opinions of their peers. For example, if a person is found to report about an incident (e.g., a robbery) in a neighborhood in a social networking website, their friends might inadvertently re-post their observations (e.g., retweet or share). Often times people tend to post rumors or falsified facts, which their followers might re-post. Such ``follower" practices thereby injects observation biases and increases the frequency of misinformation in the knowledge extracted from social data platforms. If social signals are used to locate critical events and drive mobile physical sensors (e.g., robots), the mobile agents might be unnecessarily dispatched to the wrong locations, depleting useful resources. }%On the positive side, when people report their observations online, their ``followers" might also be encouraged to report their own observations tii, thereby increasing reporting activities. 

%\mt{Thus, characterizing and determining the dependency between peers in social data platforms in SPS can potentially eliminate biases and also help to increase the quality of contributed knowledge. In contrast to social sensors which predominantly consists of humans, the deployment complexity and cost of physical sensors might require excessive manual effort and financial provisions. In SPS applications with scarce resource availability and budget constrained, such deployment complexity and cost might not be feasible. If the spatiotemporal correlations between the social and physical data can be identified and subsequently derived, they can be used to potentially lower the burden from physical sensors. For example, in the contact tracing application in Figure~\ref{fig:block}, if a strong spatiotemporal correlation in identified between the data provided by the wearable sensors and the people's posts on social media platforms, the number of required wearable sensors could be reduced.}

%\mt{While using such spatiotemporal correlations provide greater efficiency in the deployment of SPS applications, studying such intricate correlations across data form two distinct sensing domains is not a trivial task. It requires careful scrutiny of the data and accurate data provenance approaches. Identifying and characterizing the spatiotemporal correlations presents an unprecedented challenge in SPS since both temporal and spatial correlations are highly volatile and no prior knowledge is available as starting points for these correlations. Existing research has not extensively studied the extraction of spatiotemporal correlations in the context of integrated social and physical sensing in SPS.}

%Understanding the dependency between peers in social data platforms in SPS can potentially eliminate biases and increase the quality of contributed knowledge.




%evolving truthfulness of reports~\citep{zhang2017towards}, diversity of events~\citep{fan2018system}, and reliability of sources~\citep{sandhu2019social} and studies on physical sensing have proposed solutions to minimize the effect of real-world dynamics such as deadlines, communication, and energy consumption~\citep{pulido2004constraint,gu2016hed,radgi2013uav}. Regardless of their virtues, such standalone approaches are deficient in addressing the interconnected dynamism injected by the constantly evolving social media and the unpredictable physical world. } 

%: i) a more uncertain location, ii) a location with tighter deadline, or iii) a closer location. 

%false alarms leading rescue teams to veer away from potential survivors during a crucial rescue operation.} %it is difficult for SPS applications that leverage mobile physical sensors to resort to a fixed set of policies for deciding where to dispatch the mobile agents, such as cars and robots, for verifying the truthfulness of claims on social data platforms.} 

%(e.g., robots might run out of battery life) (e.g., IoT devices might lose network connectivity) (e.g., UAVs might not be able to cover an entire city in a short time)

%from the human sensors in the social data platforms. %and the physical sensors might have energy constraints (e.g., smh).

%While most WiFi implementations operate in infrastructure mode where devices communicate with each other by first going through an Access Point (AP), some instances of WiFi also operate in ad-hoc mode or mesh networks where devices communicate and exchange information without using a router~\citep{guillen2016wifi}. 

%\subsubsection{Cellular Networks}

%Bluetooth Low Energy (BLE) is a fork of the original Bluetooth standard developed by Bluetooth special interest group (SIG) to further reduce energy consumption of sensor devices while providing high-speed IP connectivity~\citep{gomez2012overview}. With the growing number of low-powered and energy-constrained sensor devices in SPS, a recent Bluetooth standard known as IEEE 802.15.4 has emerged which specifies a physical layer and a medium access control for reliable low-rate wireless personal area networks (LR-WPANs)~\citep{callaway2002home}.

%\subsubsection{Fog Computing}

%For example, in an anomaly detection with SAS application, if the uncertainty from the social signals and the captured UAV data can be determined, the uncertainties might be used as feedback signals to potentially improve the detection accuracy.} 
%However, for driving mobile physical sensors such as UAVs and cars using social media signals in SPS applications. As such it is crucial to determine the uncertainty contained in the collected data from the event report~\citep{wang2019social}. 
 %For instance, the false alarm of a forest fire can lead rescue teams to locations with no actual fire and miss out on important regions of interest.
 
 %While the above approaches have presented privacy-preserving techniques to extract data from social and physical sensors separately, they are unable to solve the privacy challenge in SPS systems where social and physical sensors deliver complementary information in a connected environment that can be exploited for exposing the personal information of the users. 
% As such, ensuring user privacy in SPS is a major difficulty due to the diversity and complementary nature of the data obtained from the various social and physical data platforms (e.g., smartphones, social media websites, and environmental sensors).}
% Beyond the purpose of sensing, personal opinions such as political views, social interactions, and daily activities conveyed through social data platforms (e.g., social media posts) might potentially be combined with relevant physical sensor metadata such as geo-location data, timestamps, and device statuses shared by users through personally-owned devices to reveal sensitive information such as ethnicity, race, and financial status. The users participating in SPS do not typically consent to sharing their personally identifiable information (PII) (e.g., online shopping habits, medical records, net worth) and such information are also not required by SPS applications~\citep{vance2018privacy}. Despite providing consent, inadvertently the sensitive information of end users might get jeopardized when information from social sensing gets combined with that from physical sensors in various SPS applications. 
%For example, in the contact tracing application of Figure~\ref{fig:block}, reports of health conditions posted by people through social media (e.g., a person having symptoms of fever) might be correlated with historical health data from wearable sensors (e.g., blood pressure, pulse rate, body temperature) to potentially infer the medical history of an individual (e.g., whether a person is suffering from a terminal illness).%(e.g., the contact tracing application in Figure~\ref{fig:block} where social media and wearable sensor data are meld together).}

%it is difficult to} establish trust among users to contribute their observations and provide access to data from their devices, which makes the privacy challenge in SPS even harder to solve. 
%It has been observed that due to the concern of private information being exposed and the potential for undesirable cases such as cyber crimes many users do not feel comfortable conveying their knowledge through social data platforms and sharing their physical sensor data. Variants of cyber crimes across social and physical sensors include: i) identity thefts (i.e., a scammer might impersonate as a real-person using that person's identifying information); ii) cyber extortion (i.e., blackmailing users with their sensitive data); and iii) cryptojacking (i.e., hackers mine cryptocurrency using computation power from other users' personal devices such as IoT devices and smartphones). As an example, in an anomalistic crowd detection application based on IoT devices (e.g., smart proximity sensors) and a crowdsensing app, the users might not feel confident installing the crowdsensing app in the first place in fear of having their identity stolen by hackers. Moreover, the users might not provide access to their homes' surveillance cameras with the concern of having their daily activities monitored~\citep{vance2018privacy}. Consequently, it is hard to develop trust among the participants in SPS applications to share their own observations and their devices' sensing data due to the privacy concerns for their personal devices. Thus, it is yet to be determined how to design robust privacy-aware SPS platforms that can foster trust among its users and address the privacy challenge in SPS.

%injected by the constantly evolving social media and the unpredictable physical world yet to be determined. %Given the unsolved dynamism challenge in SPS applications, resilient approaches that can withstand the combined dynamics from the social and physical domains is yet to be explored.

%, given the limited resources in physical sensing systems and improper decisions might affect adversely the performance of an SPS system.} %For example, during a search and rescue operation, if false reports from social media are trusted to dispatch robots without careful analysis, the true locations of the potential survivors might not be discovered on time, putting their lives at risk.}

%since it is not known how slow or fast the response of one sensing paradigm is compared to the other.

%The second hurdle is handling the highly volatile temporal and spatial correlations prevalent across the social and physical data platforms. Due to the unpredictable nature of the spatiotemporal correlations in real-world events and human sensors, it is difficult to locate their patterns and model their correlations conclusively. For example, a forest fire might or might not be correlated with visibility of smoke in a nearby city at the same time. Similarly, a person's social media post might or might not be correlated with what they posted in the past. Existing research has explored several methods to model the correlations separately in social and physical data platforms~\citep{zhang2018fauxbuster,li2007connection,kim2018development}, which mostly rely on historic data from the social and physical sensors. However, due to the presence of various dynamics in SPS applications, %which might quickly become stale in SPS applications as the correlation patterns change suddenly. 
%In addition to that, current solutions have not extensively studied methods to extract the volatile spatiotemporal correlations from the social and physical sensors in SPS. Given the transient nature of the spatiotemporal correlations across the physical and social data platforms, it is imperative to design a holistic framework that can capture the transient spatiotemporal correlations between different the sensors across social and physical sensing paradigms and connect their observations.

%\mt{On the other hand, the dynamics from the physical world might adversely impact the performance of both the social sensors and the physical sensors. For example, in a social-media-driven vehicular sensing application in the aftermath of a disaster~\citep{rashid2019socialcar}, the disaster might cause road-damage around the affected area which might potentially restrict the travel of cars. If the car drivers are unable to traverse across certain roads and intersection, they might not be able to locate and capture events of interest in the vicinity of those roads (e.g., survivors kof the disaster). Moreover, due to damage to network infrastructure in a disaster, the car drivers might lose access to network connectivity, making them unable to post any event reports. Eventually, less number of observations might be reported by the car drivers across the social media, leading to poor coverage from the human sensors. Therefore, careful consideration must be given to adapt the resource management strategy to accommodate these physical world dynamics on-the-fly, which has not been extensively explored by current literature. In the physical world, the event occurrences might also be located substantially far away from one another and might be accompanied with unforeseeable circumstances such as unfavorable weathers (e.g., hurricanes) or damaged infrastructure (e.g., roads), which might impede the physical sensing. For example, strong wind or cloud might affect the readings from different sensors such as cameras or gyroscopes on UAVs and bumpy roads might affect the sensors on vehicles. If the events are located far away from each other in the real-world, the human sensors might be slow at reporting the events on social data platforms. Moreover, if the events are located in areas unreachable to humans (e.g., inside a building after an earthquake), the social sensors might be unable to generate data all. 

%Conversely, the dynamics of the occurrences in the physical world tend to have direct impacts on the performance of the social sensing. For example, in a social-media-driven vehicular sensing application in the aftermath of a disaster~\citep{rashid2019socialcar}, the road-damage caused by a disaster might potentially restrict the travel of cars. If the car drivers are unable to traverse across certain roads and intersection, they might not be able to locate and capture events of interest in the vicinity of those roads (e.g., survivors of the disaster). Moreover, due to damage to network infrastructure in a disaster, the car drivers might lose access to network connectivity, making them unable to post any event reports. Eventually, less number of observations might be reported by the car drivers across the social media, leading to poor coverage from the human sensors. Therefore, careful consideration must be given to adapt the resource management strategy to accommodate these physical world dynamics on-the-fly, which has not been extensively explored by current literature.} 

%Motivated by the collective benefits of human-wisdom in social sensing and the empirical sensing capabilities of physical sensors, SPS is evolving as a multifaceted sensing paradigm to \mt{capture the real-world phenomenon.}%absorb vital information from the environment and  (e.g., a building on fire, an unconscious person on a roadside). %Unlike standalone sensing approaches, SPS has a more %effective information retrieval, %\mt{wider sensing scope as it harnesses the ubiquity of social sensors and also greater accuracy since it capitalizes on the empirical sensing capabilities of hardware sensors.}% and the accurate %sensing capabilities of physical sensors. 


%Through the use of wearable health-monitoring devices and remote health testing integrated with social media data, a more fine-grained representation of a patient health can be provided based on prior interactions of the person on social media expressing their health conditions (e.g., a person posting about having frequent headache could indicate potential signs of hypertension). 

 %for capturing a wide range of visual features of the objects residing on the earth's surface~\citep{zhang2018risksens,chi2017novel,rosser2017rapid,wang2018fusing,zhao2020remote,huang2017cloud}. 
 
 s~\citep{trottier2014crowdsourcing}. %provided an overview of an emerging phenomenon of how crowds can be integrated into CCTV surveillance for ALPR scheme for smart cities as well as identifying suspects involved in suspicious behaviors~\citep{trottier2014crowdsourcing}.

\mt{Prior to}

 %wearable heart rate monitors, 
 
 %transducers 
 
 %accelerometers on smartphones)
 
 %neither provide a standardized 
 %and reliable but also relatively affordable.However, regardless of their virtues 
 % since it relies on human sensors rather than hardware sensors; 
 
 %iii) biased observations since perceptions conveyed on social data platforms% are generally not as accurate as physical sensors and may be overly sensational or influenced by people's personal views and opinions, leading to poor data quality.
 
 % minimize the individual drawbacks of social and physical sensing to establish a comprehensive representation of the environment. %A few examples of such drawbacks are reliability concern of social signals, data modality limited sensing scope of physical sensors. 
 
 %\begin{figure*}[!htb]
%    \centering
   %\vspace{-0.05in}
%    \includegraphics[width=18cm]{fig/block1A.png}
%    \vspace{-0.05in}
%    \caption{Overview of Exemplary SPS Applications}
%    \vspace{-0.15in}
%    \label{fig:block}
%\end{figure*}

% illustrates a high-level overview of some representative SPS applications.%For example, in this figu %An assortment of physical sensors in the form of unmanned aerial vehicles (UAVs), vehicular sensor networks (VSN), surveillance cameras, wearable devices, and other connected devices interplay with a collection of human sensors in the social media (e.g., Twitter, Facebook) and crowdsensing platforms (e.g., Waze, AirVisual) to monitor the occurrences in the physical world. Afterward, the captured data are analyzed on backend servers or within the devices at the edge of the network to infer the state of the physical environment.

%(e.g., while monitoring a post hurricane scenario using vehicular sensors, the number of reported events in social media and their urgency may increase drastically over time, but the vehicles may be constrained by damaged roads.)}%(e.g., the number of reports in social media may evolve over time and the physical world events may have tight deadlines)?} %v) How to adapt  the ensure smooth exchange of data between the social and physical sensors vi) How to } 


%Despite great efforts being contributed towards the development of capable SPS systems, several important technical challenges still need to be addressed in order to explore the full potential of SPS: How to handle the 
%In SPS, information about the environment needs to be obtained from an ensemble of
% innumerable social and physical sensors that widely vary in terms of hardware and protocols (i.e., they are heterogeneous). 
%Thus, two challenges lie in the \textit{data collection} from the large number of sensors and the \textit{data modality and heterogeneity} due to the massive volumes of data generated by various social and physical sensors and the diversity of the involved hardware. Frequently, data in SPS applications need to be extracted from privately-owned user devices (e.g., smartphones, surveillance camera) and transmitted across networks to reach end destinations (e.g., cloud servers). Consequently, one crucial challenge in SPS is associated with ensuring \textit{security and user privacy}. In SPS, social media users constantly report incidents which may fluctuate over time and evolve with varying degrees of uncertainty~\citep{IPSN:12}. Moreover, the reported events may occur at locations far apart from one another with different levels of urgency~\citep{zhang2017constraint}. Hence, one further challenge arises from the \textit{dynamics from the social media reports and the physical world events}. Once the social media reports are used to locate events, the physical sensors are expected to work in parallel with the social media data to efficiently recover the truthful states of the incidents. As such, the last challenge in SPS is designing a closed-loop system to tightly integrate the social and physical domains. 

% (e.g., when monitoring crowds during holiday shopping, shoppers may post more frequently in the social media while motion sensors in shopping malls may also detect greater activities than normal)? %(e.g. a car driver can people in social media tend to share and follow reports of their peers)? 

% analog signals from temperature sensors)? 
%iv) How to develop a closed-loop system that seamlessly integrates the social and physical sensors to carefully coordinate the interactions between the social domain and the physical world? 
% (e.g., a person can report their illness in the social media while their wearable fitness tracker monitors their health in real-time and notifies a doctor)? %iii) How to model the human behavior and the hardware sensor characteristics (i.e., for troubleshooting failure scenarios of the sensors)? 


% (e.g., social media users may have more frequent update intervals and generate larger volumes of data than physical sensors during a crisis making it difficult to jointly locate useful data)? 
%for the present and the near future, 

%truth discovery algorithms and data analysis 

%wildfire monitoring~\citep{rashid2020compdrone}, 

%vi) How to derive the estimation accuracy and performance bounds for the detection using human cognitive models and hardware sensor parameters? 


% (e.g., after a traffic accident distinguishing between true facts and opinions in social media to determine the correct geo-location of the incident for sending a UAV to the location and assess its severity))?
%fostering trust among users to rely on an SPS-based anomaly detection system)?

%For example, in the social airborne sensing application in Figure~\ref{fig:block}, the social signals could be used to determine the location of the anomalies for sending the UAVs and afterwards the knowledge captured by the UAV sensors could be utilized to improve the social sensing by selectively discarding less reliable sources (i.e., users who continually made false claims). The design of such a closed-loop system requires a careful coordination of the interactions and communications between the HCP components. 

%You use the humans as sensors but also need to carefully control/coordinate their roles as actuators. E.g., smart water sensing. If the humans don't contribute good quality data (i.e., not enough reliable data) or the participation levels goes down, higher incentives need to be applied to provide better quality data. Here the incentives serve as control signals and the human participants perform the role of actuators. Upon receiving incentives humans might coollaborate to contribute more data, validate the data of their peers, or encourage more people to participate by referring them to use the app (i.e., take a respinse in the physical world). Such an adaptive closed loop control requires careful regulation of the incentives by using the performance of the human sensors as a feedback signal. Incentive is a signal from the cyber world (i.e., through smartphone apps) to the human world. When the humans receive the incentives, they can take an action in the physical world. Here the three components work together in one single system. How to design such a smart incentive mechanism is a unique challenge in SPS applications. This challenge is inherently different from incentive systems in particpatory sensing or crowdsensing since SPS applications involve the interactions both physical signals and social signals to bridge the loop. How to use the physical sensors to validate the information contributed by human sensors?

%Human sensors often act as rational actors and might not always take part in the sensing process. Thus, one obstacle in handling the HCP interactions in SPS is the inconsistent availability of the human sensors, known as \textit{churn}~\citep{zhang2019heteroedge}. For example, in an interesting place discovery application using crowdsensing and smartphone sensors~\citep{huang2016unsupervised}, the human participants might focus on personal goals instead of the sensing task and abandon the given assignments. This might lead to poor sensing coverage for the physical sensors such as the smartphone GPS, camera and microphone. Recent literature on distributed systems has proposed methods to mitigate churn by using reputation-based measures to allocate tasks to more reliable devices~\citep{zhang2010cloud}, increasing the total number of devices in the system~\citep{godfrey2006minimizing, haeberlen2006fallacies}, and allowing redundant allocation of critical tasks~\citep{vaquero2019research}. The above schemes can potentially minimize churn in purely physical sensor-based systems, where the churn is mainly caused by device failures and network constraints that are relatively simpler to troubleshoot. In a similar fashion, existing solutions might be able to address the churn issue in purely crowdsensing systems (e.g., Waze), where the churn occurs only due to the infrequent participation of online users without. However, with the prevalence of humans-in-the-loop in SPS applications, the churn issue is even more prominent and challenging to solve due to the interconnection between the interactions of the social and physical worlds which are inherently hard to model and predict. 

%Furthermore, various unprecedented physical world constraints can also directly impact the behavior of human sensors. For example, in a social-media-driven vehicular sensing application in the aftermath of a disaster (e.g., a hurricane)~\citep{rashid2019socialcar}, the participating car drivers might abruptly drop their assigned tasks in the middle of exploration due to concerns of safety along the road, the sensing devices in the cars (e.g., dashboard sensors) might lose internet connectivity, or the cars might run out of fuel, causing churn in the system. Consequently, current solutions are unable to solve the issue of churn in SPS applications. As such, it remains an open challenge to solve the HCP challenge prevalent in SPS systems.%in a decisive manner in SPS applications.

%in the aftermath of a disaster (e.g., a hurricane) using crowdsensing and mobile sensors. While two nearby fuel stations might not have direct connections between each other, the availability of fuel at one fuel station might be implicitly correlated to the fuel availability at its nearby fuel stations (e.g., due to their close proximity to each other or the same supplier of fuel at the stations). The implicit correlations in SPS are hard to perceive and model solely based on the sensing data obtained from the social and physical sensors. For example, in the fuel availability locator application, reports of the fuel at particular stations might not provide enough evidence to conclude on the existence of the implicit connections. 


%For example, a surveillance camera at a shopping mall can only capture the image of a person without further details of the person. However, if that particular person uses a crowdsensing app \mt{} where they periodically share their shopping history and geo-location information, the image data from the cameras might be combined with these additional data to unravel the socioeconomic status of the individual.

% In SPS applications the rate and pattern of information generation is different between the social and physical sensors. For example, human sensors are more likely to be triggered by real-world stimuli and might take a while to respond to happenings around them and tend to only generate reports during significant occurrences (e.g, posting of Tweets during a sudden crowd gathering). During the course of such significant occurrences, the frequency of activities across social data platforms might increase drastically~\citep{wang2019age}, causing a bursting/spiking pattern of data. On the other hand, physical sensors are more likely to generate data in real-time without any delays and constant rate (e.g., live regular stream of video from surveillance cameras). Regardless of the existence of major real-world occurrences, physical sensors are designed to constantly capture the real-world phenomenon. In an SPS system, incorporating such dynamic information generation characteristics of social and physical sensors is a non-trivial task.

% The dynamic information generation phenomenon of social and physical sensors might also lead to uncertain correlation windows. \mt{The speed of data generation by social sensors are inherently different from physical sensors. For example, let us consider a damage assessment application using social vehicular sensor network (S-VSN). The rate at which vehicular sensors like dashboard cameras capture images differs from the frequency at which the car drivers report damage in social media. The car drivers are more likely to be triggered by real-world stimuli, taking a while to respond to happenings around them while the vehicular sensors generate data at periodic intervals. If the damage status of a place changes from no damage to severe damage over time, the delay of the sensing measurements between the human sensors and vehicular sensors might vary, leading to a situation of correlated dynamism. } Recent studies on social sensing have developed methods to model the dynamics across social data platforms such as scalable streaming truth discovery~\citep{zhang2017towards}, online learning-driven topic discovery~\citep{pandharipande2020social}, and reputation-based source pruning~\citep{sandhu2019social}. In a similar fashion, studies on physical sensing have proposed solutions to extensively model the dynamics from the physical world such as particle swarm optimization~\citep{pulido2004constraint}, mixed integer linear programming~\citep{yin2017dynamic}, and cycle chain algorithms~\citep{li2014modeling}. While the above solutions could potentially help to explore the dynamics in the social and physical worlds individually, they are unable to address the correlated dynamism prevalent in SPS applications. \mt{The delay between the human and physical sensors might be uncertain and transient (i.e., varying over time). Given the dynamic and uncertain nature of the correlation window, it is difficult to compute the correlation between social sensing measurements and that of physical sensing.}  

%The speed of data generation by social sensors are inherently different from physical sensors (e.g.,,the rate at which UAVs capture images is different from the frequency at which people report anomalous incidents in social media). Let us,


%While SPS imposes new challenges for researchers, it also paves the road for future work at the intersection of the cyber, social, and physical realms.}







%With the advent of human-centric sensing and the rich raw-data capture capabilities of physical sensors, social-physical sensing (SPS) is gradually protruding as a versatile sensing paradigm that leverages the complementary aspects of social sensing (i.e., social media, crowdsensing) and physical sensing (e.g., camera, GPS) for reliable information retrieval. Since SPS exploits the collective strengths of both social ``signals" which are pervasive and physical sensors which have relatively high accuracy, it delivers a more effective sensing performance compared to standalone approaches, especially in critical applications such as anomaly detection and disaster response. In this survey paper, we provide a comprehensive study of SPS, with an emphasis on its key drivers, definition, research challenges, representative applications, and potential future research directions. We start by discussing the essential motivation behind integrating the domains of social sensing and physical sensing in SPS. We then provide an overview and generalized definition of SPS. Subsequently, we highlight the key enabling technologies that serve as the basic premise for SPS. We identify the potential challenges in designing robust SPS schemes. Afterward, we identify the various paradigms driven by SPS and discuss the state-of-the-art works. Finally, we highlight a few research directions and avenues for future work in SPS.

% , maturing into an established sensing paradigm that capitalizes on the raw-data capture properties of physical sensors.
% such as vehicular and smartphone sensors and wireless sensor networks %(e.g., vehicular sensors, surveillance camera, smartphone GPS) to capture the real-world phenomena. 


%. Despite its swiftness, reliability, and accuracy in perceiving physical world stimuli with high fidelity,

 %search and rescue operations, 
 
 %such as multifaceted sensing, greater mobility and wider sensing scope , 

 \addtocounter{table}{-1}         
          
 \begin{table}[htb!]
     \caption{List of Abbreviations and Acronyms (continued)}
     \center
     \begin{tabular}{|l|l|}
         \hline
         \centering          
          
          
     \end{tabular}
     \label{tab:definition1}
 \end{table}
 

